MAHALO: Unifying Offline Reinforcement Learning and Imitation Learning from Observations

We study a new paradigm for sequential decision making, called offline policy learning from observations (PLfO). Offline PLfO aims to learn policies using datasets with substandard qualities: 1) only a subset of trajectories is labeled with rewards, 2) labeled trajectories may not contain actions, 3) labeled trajectories may not be of high quality, and 4) the data may not have full coverage. Such imperfection is common in real-world learning scenarios, and offline PLfO encompasses many existing offline learning setups, including offline imitation learning (IL), offline IL from observations (ILfO), and offline reinforcement learning (RL). In this work, we present a generic approach to offline PLfO, called $\textbf{M}$odality-agnostic $\textbf{A}$dversarial $\textbf{H}$ypothesis $\textbf{A}$daptation for $\textbf{L}$earning from $\textbf{O}$bservations (MAHALO). Built upon the pessimism concept in offline RL, MAHALO optimizes the policy using a performance lower bound that accounts for uncertainty due to the dataset's insufficient coverage. We implement this idea by adversarially training data-consistent critic and reward functions, which forces the learned policy to be robust to data deficiency. We show that MAHALO consistently outperforms or matches specialized algorithms across a variety of offline PLfO tasks in theory and experiments. Our code is available at https://github.com/AnqiLi/mahalo.

==> tables/d4rl_results.tex <==
\begin{table*}[t]
\caption{Results on D4RL benchmark~\cite{fu2020d4rl} We show the average normalized score across 3 random seeds. Algorithms with scores greater than 0.9 of the best score (excluding Oracle) is marked in bold. MAHALO achieves top performance in almost every scenario and task except halfcheetah. MAHALO is also able to match Oracle performance, despite having access to less reward data. $^-$ ATAC only uses data with both dynamics and reward information. $^*$ BC and BCO does not use expert reward. $^+$ Oracle has access to reward for all dynamics data.}
\label{tab:mujoco}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
\toprule
Scenario & Dataset & MAHALO & RP & AP & UDS &  UDS-A & ATAC$^\dagger$ & BCO$^*$ & BC$^*$ & Oracle$^+$ \\ 
\hline
ILfO & hopper & \textbf{107.85} & \textbf{97.91} & 59.73 & - & - & - & 54.28 & - & - \\ 
 & walker & \textbf{87.31} & 78.54 & 57.20 & - & - & - & 50.76 & - & - \\ 
 & halfcheetah & \textbf{62.89} & 34.14 & 5.49 & - & - & - & 5.67 & - & - \\ 
\hline
IL & hopper & \textbf{104.27} & \textbf{97.56} & 58.90 & 34.29 & 29.48 & 79.62 & - & 33.26 & - \\ 
 & walker & \textbf{89.75} & 77.05 & 79.62 & 4.31 & 4.27 & \textbf{81.30} & - & 28.54 & - \\ 
 & halfcheetah & \textbf{59.88} & 28.58 & 6.35 & 20.38 & 25.57 & 5.53 & - & 20.28 & - \\ 
\hline
RLfO & hopper & \textbf{107.04} & \textbf{107.79} & 60.15 & - & - & - & 54.28 & - & 107.82 \\ 
 & walker & \textbf{104.40} & \textbf{98.40} & 66.83 & - & - & - & 50.76 & - & 98.21 \\ 
 & halfcheetah & 57.39 & \textbf{69.58} & 2.92 & - & - & - & 5.67 & - & 61.39 \\ 
\hline
RL-expert & hopper & \textbf{110.68} & \textbf{105.94} & 65.19 & 98.52 & 97.26 & 64.15 & - & 33.26 & 107.82 \\ 
 & walker & \textbf{110.10} & 98.48 & 66.99 & 74.66 & 74.48 & 84.86 & - & 28.54 & 98.21 \\ 
 & halfcheetah & 40.47 & \textbf{63.48} & 4.09 & 7.34 & 9.15 & 2.42 & - & 20.28 & 61.39 \\ 
\hline
RL-sample & hopper & \textbf{107.62} & \textbf{105.40} & 72.07 & 0.96 & 0.92 & 91.44 & - & - & 107.30 \\ 
 & walker & \textbf{95.47} & \textbf{94.65} & 2.86 & -0.01 & 0.00 & 6.79 & - & - & 96.34 \\ 
 & halfcheetah & \textbf{68.77} & \textbf{70.24} & 11.35 & 24.06 & 19.89 & 17.53 & - & - & 68.44 \\ 
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}

==> tables/fixed_beta_d4rl_results.tex <==
\begin{table*}[t]
\color{blue}
\caption{Results on D4RL benchmark~\cite{fu2020d4rl}. We show the average normalized score over 50 evaluation trials across 10 random seeds. Algorithms with scores greater than 0.9 of the best score (excluding Oracle) is marked in bold. MAHALO achieves top performance in almost every scenario and task except halfcheetah. MAHALO is also able to match Oracle performance, despite having access to less reward data. We use a \emph{fixed} $\beta=10.0$ for {all ATAC-based algorithms across all experiments}, including MAHALO, RP, AP, UDS, UDS-A, ATAC and Oracle. We use a \emph{fixed} $\alpha=1000000.0$ for MAHALO. $^-$ ATAC only uses data with both dynamics and reward information. $^*$ BC, BCO and SMODICE does not use expert reward. $^+$ Oracle has access to reward for all dynamics data. }
\label{tab:mujoco-fixed-beta}
\begin{center}
\begin{small}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c||c}
\toprule
Scenario & Dataset & MAHALO & RP & AP & UDS &  UDS-A & ATAC$^\dagger$ & BCO$^*$ & BC$^*$ & {\tiny SMODICE$^*$} & Oracle$^+$ \\ 
\hline
ILfO & hopper & \textbf{104.66} & \textbf{95.66} & 45.97 & - & - & - & 46.80 & -  & 59.80 & - \\ 
 & walker & \textbf{87.97} & 77.15 & 61.11 & - & - & - & 63.02 & - & 4.57 & - \\ 
 & halfcheetah & {28.16} & 18.26 & 3.70 & - & - & - & 5.16 & - & \textbf{57.02} & - \\ 
\hline
IL & hopper & \textbf{104.06} & \textbf{95.46} & 45.93 & 22.42 & 22.05 & 62.08 & - & 32.12 & 69.77 & - \\ 
 & walker & \textbf{89.03} & 77.71 & 63.53 & 3.23 & 2.76 & 70.40 & - & 18.78 & 4.46 & - \\ 
 & halfcheetah & {34.12} & 19.74 & 3.74 & 17.58 & 18.24 & 3.64 & - & 22.36 & \textbf{52.88} & - \\ 
\hline
RLfO & hopper & \textbf{95.31} & \textbf{100.83} & 40.58 & - & - & - & - & - & - & 101.06 \\ 
 & walker & \textbf{94.65} & \textbf{96.91} & 52.35 & - & - & - & - & - & - & 97.82 \\ 
 & halfcheetah & \textbf{31.79} & 25.11 & 3.35 & - & - & - & - & - & - & 21.22 \\ 
\hline
RL-expert & hopper & \textbf{84.02} & \textbf{83.24} & 34.93 & 67.51 & 54.54 & 51.14 & - & - & - & 101.06 \\ 
 & walker & \textbf{103.18} & \textbf{98.31} & 50.03 & 71.92 & 65.18 & 60.76 & - & - & - & 97.82 \\ 
 & halfcheetah & \textbf{25.87} & \textbf{27.86} & 1.73 & 13.68 & 8.04 & 2.60 & -  & - & - & 21.22\\ 
\hline
RL-sample & hopper & \textbf{84.98} & \textbf{90.12} & 71.92 & 0.81 & 0.81 & 56.58 & - & - & - & 93.19 \\ 
 & walker & \textbf{93.48} & \textbf{93.98} & -0.02 & -0.09 & -0.09 & -0.11 & - & - & - & 93.59 \\ 
 & halfcheetah & \textbf{27.52} & \textbf{25.70} & 13.26 & 7.11 & 9.92 & 17.58 & - & - & - & 28.83 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}

\begin{table*}[t]
\color{blue}
\caption{Success rate on Meta-World~\cite{yu2020meta}. The success rate is computed over 50 evaluation episodes. We consider an episode success if it is able to reach the goal within $128$ steps. We report the average success rate across 10 random seeds. MAHALO is one of the overall best-performing algorithms. ATAC also achieves strong results in IL and RL-expert because it is presented with expert-only data. We use a \emph{fixed} $\beta=10.0$ for all ATAC-based baselines, including MAHALO, RP, AP, UDS, UDS-A, ATAC and Oracle. We use a \emph{fixed} $\alpha=1000.0$ for MAHALO. }
\label{tab:mw-fixed-beta}
\begin{center}
\begin{small}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
\toprule
Scenario & Dataset & MAHALO & RP & AP & UDS &  UDS-A & ATAC$^\dagger$ & BCO$^*$ & BC$^*$ & Oracle$^+$ \\ 
\hline
ILfO & reach & \textbf{61.8} & \textbf{62.6} & 8.8 & - & - & - & 13.5 & - & - \\ 
 & push & \textbf{47.2} & 2.8 & 12.4 & - & - & - & 16.0 & - & - \\ 
 & plate-slide & \textbf{97.4} & 0.0 & 75.8 & - & - & - & 84.0 & - & - \\ 
 & handle-press & 23.8 & 17.2 & \textbf{88.4} & - & - & - & 79.5 & - & - \\ 
 & button-press & \textbf{81.6} & 11.2 & \textbf{82.0} & - & - & - & \textbf{86.5} & - & - \\ 
\hline
IL & reach & 22.0 & 11.6 & 35.4 & 8.8 & 0.2 & \textbf{89.4} & - & 58.5 & - \\ 
 & push & \textbf{92.6} & 4.4 & 30.0 & 79.2 & 57.2 & 30.8 & - & \textbf{93.5} & - \\ 
 & plate-slide & 80.4 & 0.0 & \textbf{89.8} & 74.4 & 54.8 & 57.8 & - & 80.5 & - \\ 
 & handle-press & 36.2 & 29.6 & \textbf{100.0} & 23.0 & 57.4 & 80.4 & - & 82.0 & - \\ 
 & button-press & \textbf{100.0} & 79.2 & 88.8 & \textbf{100.0} & \textbf{99.8} & 74.0 & - & \textbf{100.0} & - \\ 
\hline
RLfO & reach & \textbf{83.6} & \textbf{88.0} & 15.0 & - & - & - & - & - & 51.0 \\ 
 & push & \textbf{56.8} & 28.6 & 12.8 & - & - & - & - & - & 91.8 \\ 
 & plate-slide & \textbf{99.8} & \textbf{100.0} & 68.4 & - & - & - & - & - & 99.2 \\ 
 & handle-press & 77.8 & 84.4 & \textbf{96.0} & - & - & - & - & - & 54.0 \\ 
 & button-press & \textbf{99.6} & \textbf{100.0} & 82.8 & - & - & - & - & - & 100.0 \\ 
\hline
RL-expert & reach & 35.2 & 48.6 & 42.0 & 33.2 & 33.6 & \textbf{97.2} & - & - & 51.0 \\ 
 & push & \textbf{92.0} & \textbf{86.6} & 22.6 & \textbf{85.4} & \textbf{83.8} & 62.2 & - & - & 91.8 \\ 
 & plate-slide & \textbf{97.4} & \textbf{100.0} & 83.6 & \textbf{99.4} & \textbf{99.0} & 70.8 & - & - & 99.2 \\ 
 & handle-press & 62.4 & 69.8 & \textbf{88.4} & 77.2 & 64.4 & \textbf{89.0} & - & - & 54.0 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{92.6} & \textbf{100.0} & \textbf{98.4} & \textbf{90.0} & - & - & 100.0 \\ 
\hline
RL-sample & reach & \textbf{86.0} & \textbf{87.4} & 57.8 & \textbf{87.4} & \textbf{89.8} & \textbf{85.4} & - & - & 88.8 \\ 
 & push & 40.6 & \textbf{45.2} & 20.8 & 35.8 & 34.6 & 35.0 & - & - & 39.2 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & \textbf{97.0} & \textbf{95.8} & \textbf{90.0} & \textbf{97.4} & - & - & 100.0 \\ 
 & handle-press & 69.4 & 81.0 & \textbf{100.0} & 76.8 & 75.8 & 53.6 & - & - & 79.0 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & - & 100.0 \\ 
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}

==> tables/mw_results.tex <==
\begin{table*}[t]
\caption{Success rate on Meta-World~\cite{yu2020meta}. The success rate is computed over 50 evaluation episodes. We consider an episode success if it is able to reach the goal within $128$ steps. We report the average success rate across 3 random seeds. MAHALO is one of the overall best-performing algorithms. ATAC also achieves strong results in IL and RL-expert because it is presented with expert-only data.}
\label{tab:mw-rewards}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c||c}
\toprule
Scenario & Dataset & MAHALO & RP & AP & UDS &  UDS-A & ATAC$^\dagger$ & BCO$^*$ & BC$^*$ & Oracle$^+$ \\ 
\hline
ILfO & reach & \textbf{64.7} & \textbf{62.7} & 16.7 & - & - & - & 16.5 & - & - \\ 
 & push & \textbf{68.7} & 7.3 & 20.0 & - & - & - & 18.0 & - & - \\ 
 & plate-slide & \textbf{100.0} & 13.3 & \textbf{98.7} & - & - & - & 82.5 & - & - \\ 
 & handle-press & \textbf{91.3} & 36.0 & \textbf{97.3} & - & - & - & 86.5 & - & - \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{93.3} & - & - & - & 89.5 & - & - \\ 
\hline
IL & reach & 58.0 & 17.3 & 42.0 & 16.7 & 2.7 & \textbf{98.7} & - & 33.5 & - \\ 
 & push & \textbf{92.0} & 24.0 & 48.7 & 82.0 & 76.7 & 66.7 & - & 40.5 & - \\ 
 & plate-slide & \textbf{96.0} & 16.7 & 88.7 & 62.7 & 88.7 & \textbf{100.0} & - & 69.5 & - \\ 
 & handle-press & 62.7 & 48.0 & \textbf{100.0} & 44.0 & 46.7 & \textbf{100.0} & - & 79.5 & - \\ 
 & button-press & \textbf{100.0} & \textbf{99.3} & \textbf{98.7} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 88.5 & - \\ 
\hline
RLfO & reach & \textbf{87.3} & \textbf{90.7} & 14.0 & - & - & - & 16.5 & - & 58.0 \\ 
 & push & \textbf{67.3} & 36.7 & 18.7 & - & - & - & 18.0 & - & 90.0 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & \textbf{91.3} & - & - & - & 82.5 & - & 100.0 \\ 
 & handle-press & 77.3 & 89.3 & \textbf{100.0} & - & - & - & 86.5 & - & 86.0 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{93.3} & - & - & - & 89.5 & - & 100.0 \\ 
\hline
RL-expert & reach & 64.0 & 62.0 & 46.0 & 63.3 & 84.7 & \textbf{98.7} & - & 33.5 & 58.0 \\ 
 & push & \textbf{94.7} & 88.0 & 35.3 & \textbf{94.0} & \textbf{94.7} & \textbf{100.0} & - & 40.5 & 90.0 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & \textbf{97.3} & \textbf{100.0} & \textbf{99.3} & \textbf{92.0} & - & 69.5 & 100.0 \\ 
 & handle-press & 76.0 & 84.7 & \textbf{100.0} & 82.0 & 82.0 & \textbf{99.3} & - & 79.5 & 86.0 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{98.7} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & 88.5 & 100.0 \\ 
\hline
RL-sample & reach & \textbf{84.7} & \textbf{92.0} & 58.7 & \textbf{91.3} & \textbf{86.0} & \textbf{84.0} & - & - & 92.0 \\ 
 & push & \textbf{48.0} & \textbf{45.3} & 16.7 & 32.0 & 32.7 & 21.3 & - & - & 48.0 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & \textbf{95.3} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & - & 100.0 \\ 
 & handle-press & 84.7 & 86.7 & \textbf{100.0} & 88.7 & 84.0 & 82.0 & - & - & 80.7 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & - & 100.0 \\
 \bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}

==> tables/new_mw_results_copy.tex <==
\begin{table*}[t]
\color{blue}
\caption{Success rate of the final policy (with the exception of SMODICE$^*$) on Meta-World~\cite{yu2020meta}. The success rate is computed over 50 evaluation episodes. We consider an episode success if it is able to reach the goal within $128$ steps. We report the average success rate across 10 random seeds. MAHALO is one of the overall best-performing algorithms. ATAC also achieves strong results in IL and RL-expert because it is presented with expert-only data. % $^*$ SMODICE is not able to train reliably, and often diverges during training. We therefore take the success rate of the best performing policy during training instead of the final one.
}
\label{tab:mw-rewards}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c||c}
\toprule
Scenario & Dataset & MAHALO & RP & AP & UDS &  UDS-A & ATAC$^\dagger$ & BCO & BC & {\tiny SMODICE} & Oracle$^+$ \\ 
\hline
ILfO & reach & \textbf{65.0} & \textbf{62.6} & 13.0 & - & - & - & 13.5 & - & 58.4 & - \\ 
 & push & \textbf{62.4} & 11.6 & 12.4 & - & - & - & 16.0 & - & \textbf{62.2} & - \\ 
 & plate-slide & \textbf{100.0} & 22.0 & \textbf{94.0} & - & - & - & 84.0 & - & \textbf{99.8} & - \\ 
 & handle-press & 75.4 & 32.4 & \textbf{96.6} & - & - & - & 79.5 & - & \textbf{98.0} & - \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{93.6} & - & - & - & 86.5 & - & \textbf{99.2} & - \\ 
\hline
IL & reach & 24.6 & 23.6 & 38.0 & 21.6 & 13.6 & \textbf{98.0} & - & 58.5 & 61.4 &  - \\ 
 & push & \textbf{92.6} & 11.8 & 35.2 & 79.2 & 72.4 & 50.0 & - & \textbf{93.5} & 65.0 & - \\ 
 & plate-slide & 80.4 & 34.4 & {89.8} & 76.2 & 62.0 & {89.4} & - & 80.5 & \textbf{100.0} & - \\ 
 & handle-press & 71.4 & 34.8 & \textbf{100.0} & 35.2 & 57.4 & \textbf{97.0} & - & 82.0 & \textbf{98.4} & - \\ 
 & button-press & \textbf{100.0} & \textbf{99.8} & \textbf{96.2} & \textbf{100.0} & \textbf{100.0} & \textbf{99.6} & - & \textbf{100.0} & \textbf{100.0} & - \\ 
\hline
RLfO & reach & \textbf{86.4} & \textbf{88.0} & 15.0 & - & - & - & - & - & - & 51.6\\ 
 & push & \textbf{58.2} & 32.0 & 20.2 & - & - & - & - & - & - & 91.8 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & 83.2 & - & - & - & - & - & - & 100.0\\ 
 & handle-press & 77.8 & 84.4 & \textbf{96.0} & - & - & - & - & - & - & 78.6 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{92.6} & - & - & - & - & - & - & 100.0 \\ 
\hline
RL-expert & reach & 39.2 & 54.0 & 42.0 & 57.8 & 33.6 & \textbf{98.4} & - & - & - & 51.6 \\ 
 & push & \textbf{95.6} & 88.6 & 40.4 & \textbf{90.4} & \textbf{90.0} & \textbf{99.6} & - & - & - & 91.8 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & 89.6 & \textbf{99.4} & \textbf{99.0} & 85.4 & - & - & - & 100.0 \\ 
 & handle-press & 72.6 & 82.0 & \textbf{97.6} & 81.2 & 80.8 & \textbf{99.0} & - & - & - & 78.6 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{97.0} & \textbf{100.0} & \textbf{100.0} & \textbf{96.4} & - & - & - & 100.0 \\ 
\hline
RL-sample & reach & \textbf{86.6} & \textbf{87.4} & 63.0 & \textbf{87.4} & \textbf{89.8} & \textbf{85.4} & - & - & - & 88.8 \\ 
 & push & 40.6 & \textbf{47.8} & 29.2 & 35.8 & 37.4 & 35.0 & - & - & - & 46.0 \\ 
 & plate-slide & \textbf{100.0} & \textbf{100.0} & \textbf{97.6} & \textbf{100.0} & \textbf{100.0} & \textbf{99.6} & - & - & - & 100.0 \\ 
 & handle-press & 78.4 & 81.0 & \textbf{100.0} & 76.8 & 77.8 & 82.8 & - & - & - & 83.4 \\ 
 & button-press & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & - & - & - & 100.0 \\ 
 \bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
